The Fragility of Fairness: Causal Sensitivity Analysis for Fair Machine Learning

Fairness metrics are a core tool in the fair machine learning literature (FairML), used to determine that ML models are, in some sense, "fair". Real-world data, however, are typically plagued by various measurement biases and other violated assumptions, which can render fairness assessments meaningless. We adapt tools from causal sensitivity analysis to the FairML context, providing a general framework which (1) accommodates effectively any combination of fairness metric and bias that can be posed in the "oblivious setting"; (2) allows researchers to investigate combinations of biases, resulting in non-linear sensitivity; and (3) enables flexible encoding of domain-specific constraints and assumptions. Employing this framework, we analyze the sensitivity of the most common parity metrics under 3 varieties of classifier across 14 canonical fairness datasets. Our analysis reveals the striking fragility of fairness assessments to even minor dataset biases. We show that causal sensitivity analysis provides a powerful and necessary toolkit for gauging the informativeness of parity metric evaluations. Our repository is available here: https://github.com/Jakefawkes/fragile_fair.

==> biases/ecd.tex <==
\section{Extra-Classificatory Decisions}

A major department store boasts a sandwich board sign at its entrance advertising diamond wedding rings. The sign reads in English on one side, in Spanish, on the other. The financing structures offered for the rings differ depending on what side of the sign you are on. Unsurprisingly, the discrepancy in financing structures does not favour the Spanish speaker. It is well known that companies are less likely to open credit lines for women, less likely to grant mortgages to blacks, less likely to grant loans to hispanics. It is less widely appreciated that the \textit{rate} at which loans, mortgages, and credit lines are granted exhibit such demographic discrepancies as well. This matters. If black people are given worse mortgage rates which are harder to repay, they will on average repay their loans at lower rates. This will be reflected in the data the company trains on in the future, hence lending apparent empirical support to those very lending policies which penalise racial minorities and make it difficult for them to repay loans. Such \textit{extra-classificatory decisions} are never factored into the models companies use to make lending determinations, nor in company internal or external evaluations of whether or not such determinations have been discriminatory. Extra-classificatory decisions are not limited to loan and interest rates. At the more concrete and transparent end of the spectrum, you have such decisions as loan and interest rates, salaries, and bail amounts. More indirect, but no less relevant, are things like employee or student resources, discrimination and sexual harassment policies, and cohort effects. Performance and retention of indigenous college students will be highly dependent on the presence of other indigenous students and the existence of financial, mentoring, and community resources. Women perform better at their jobs when they do not face sexual assault and harassment or, if and when they do, they have functioning institutional recourse to address it. 

Though such extra-classificatory decisions exist fully under the control of the deployers/decision makers, and are empirically known to be outcome-determining difference-makers for the classified populations, outcome-dependent fairness notions will be agnostic to them. Banks can lend to black loan or mortgage requesters at only rates that are prohibitive to them paying them back while granting good and managable rates to white loan requesters and then utilise the inability of black loan requesters to justify continuing to deny loans to black loan requesters or upholding differential interests rates. 

This is perhaps easiest to visualise in a causal setting. Take a set of nodes that are 100\% under the control of the firm/lending agent/decision-maker/deployer, meaning that they can set these arbitrarily. If the firm has the ability to set any of these in such a way that a single demographic is prohibited from benefitting from the firm’s decisions (???), this must be a factor in the determination of the firm’s “fairness” in decision-making. 


The conceptual incoherence of outcome-dependent fairness metrics flows from the fact that these metrics \textit{affirm the rights of firms to disparate treatment of demographic categories so long as this disparate treatment appears to find support in the observational data}. The critical point here is that there are myriad ways in which such empirical support can be \textit{engineered by firms} in their control of a slew of outcome-swamping variables beyond the single classificatory decisions evaluated under statistical fairness metrics. 


Outcome-dependent notions of fairness, the predominating metrics in the fairness literature subsequent to the publication of the equalised odds paper \cite{hardt2016equality}, define fairness relative to an estimate of the accuracy of the classifier. Such an estimate (implicitly) invokes access to a risk score which, in practice, we cannot actually observe. This risk score (and therefore the whole procedure) encapsulates uncertainty over the classifier under the assumption that the classification itself is the only degree of freedom---all else is held fixed. This may seem to be a reasonable idealisation over a statistical inference procedure---in general, it is---but when imported into a fairness context it loses coherence. 

==> examples/employment.tex <==
I am a software company in the Bay Area and I hire an equal number of men and women to junior dev positions but offer the men 200K start and the women 50K start. The men perform well at the job because 200K is sufficient to cover the cost of living in the Bay Area. The women are forced to work half of their time driving for rideshare companies or waiting tables because they have not been given a salary capable of covering the local cost of living. Consequently, they underperform. Outcome-dependent fairness notions allow me to to look at the performance of different demographic groups as solely a product of the decision point of whom to \textit{hire}. I am then able to justify hiring men and women at differential rates (or offering different introductory salaries) by dint of the observed demographic performance discrepancies. But, as we have seen, I, the firm, have \textit{manufactured these demographic performance discrepancies}. 

\nic{Proxy labels and cohort effects ?}

==> examples/lending.tex <==


\nic{selection and confounding?}

==> main/abstract.tex <==

\begin{abstract}
    %An expansive literature on ML fairness exists by now, with questionable efficacy at actually remediating or preventing bias stemming from ML systems deployed uncarefully in socially-sensitive contexts. One of the most useful things technologists can contribute to that end is providing tools for auditors and regulators to determine whether discrimination has occurred in a deployed ML system. The intricacies of real-world deployment dynamics make this task especially hard and, to date, very little technical machinery exists to carry it out effectively. In particular, the difficulties of obtaining any statistical guarantees under stacked selection procedures are considered. To this end, we put forward several results on testing procedures in order to guarantee fairness under various classes of fairness definitions, understood as constraints on an optimisation procedure. The three classes of definitions we evaluate are statistical parity, individualised, outcome-independent fairness definitions, and causal definitions. We investigate the quantity of randomised draws needed to ensure fairness under various definitions and contributions of classifier function class to this determination. We further investigate the prospect of discriminatory outcomes for classified individuals beyond the moment of classification. Stretching the three evaluated classes of fairness definitions to accommodate these post-classification scenarios reveals the conceptual incoherence of outcome-independent fairness definitions. 
    
    %When auditing and evaluating fair machine learning models, practitioners often have to sacrifice what they want to measure for a substitute based on available data. This leaves them evaluating a variety of disparity metrics on incorrect populations, using poor measurements of a "true outcome", and unable to take the causal impact of firms' additional decisions into account. Inspired by this problem, we develop a practical sensitivity analysis tool that allows regulators to understand how robust their disparity evaluations are to each of these data quality concerns. Our framework  leverages tools from causal sensitivity analysis. Auditors must specify some assumptions on the causal structure and severity of the bias and they can then assess the fragility of their conclusions to statistical biases.  
    %To demonstrate the effectiveness of our approach, we use it to evaluate the sensitivity of numerous predictors trained on a variety of ML fairness datasets, drawing conclusions on comparative robustness of parity metrics to different forms of statistical biases.


    %The machine learning ethics literature has concentrated for much of its duration on the production of tools for guaranteeing the “fairness” of ML-based tools. “Fairness,” in this context, has classically been understood as a property of a trained model in a vacuum. We demonstrate that the satisfaction of parity constraints is always dependent upon a variety of contextual factors, including choice of proxy label, reference population, and the causal structure of the problem space including classifier-imposed policies. We introduce a typology of model biases, giving them a rigorous characterisation within a causal setting and illustrating them by example. “Fairness,” we show, breaks down when biases are introduced along any number of these dimensions. In light of this, we develop tools from causal sensitivity analysis for the detection of this range of biases. These we bring together into a unified framework for regulators to test and audit models. This framework has the benefit of being parity metric agnostic and unencumbered by simplifying probabilistic assumptions. We demonstrate the efficacy of our approach in employing it to evaluate the sensitivity of numerous classifiers trained on a variety of benchmark fairness datasets. From this we are able to draw conclusions on the prevalence of the outlined bias types and the comparative robustness of various forms of parity metric to different forms of statistical bias.

% The fair machine learning literature has produced a number of disparity metrics which practitioners use to certify that ML models are in some sense "fair".  We show how this procedure relies on a number of hidden assumptions which are almost never satisfied in the real world settings. In practice the data available are often from the wrong population (selection bias), data on demographics and outcomes can be incorrect (proxy bias), and firms often causally effect outcomes via extra-classificatory decicions. Each of these problems render standard practices unsuited to the regulatory context. Using tools from causal inference we develop a general sensitivity analysis framework regulators can use to understand how robust their disparity evaluations are to these kinds of statistical bias. 
% We conduct empirical analyses using common fair ML datasets demonstrating these are not theoretical issues: many seemingly fair ML models are \textit{fragile}. Small violations of the core assumptions in disparity testing lead models with no/small disparities to have large disparities. Furthermore our analysis reveals that  disparity metrics are differentially sensitive to different kinds of bias. Causal sensitivity analysis will allow regulators to understand how these dynamics unfold in their particular circumstances for the disparity measures they are interested in.

The fair machine learning literature (FairML) produces metrics 
which are applied to certify that ML models are, in some sense, “fair.”  However when evaluating these metrics, practitioners are often left with data that is insufficient to correctly estimate these statistics, due to a variety of measurement biases and assumption violations. To name a few such issues,
(i) data on outcomes is often noisy (proxy bias);
(ii) available data are often drawn from the wrong population (selection bias);
and (iii) firms often causally impact outcomes via extra-classificatory policies. Motivated by these problems, we develop a general framework for automated sensitivity analysis in FairML settings by applying tools from causal inference.  This framework allows auditors to flexibly specify different kinds and combinations of measurement bias, along with other domain specific assumptions, to understand the robustness of their parity metrics.

is well known that this procedure relies on a number of hidden assumptions 
almost never satisfied in real-world deployment settings. 
In practice, 
(i) data on both demographics labels and outcomes can be noisy (proxy bias);
(ii) available data are often drawn from the wrong population (selection bias);
and (iii) firms often causally impact outcomes via extra-classificatory policies, among other important data issues.
% Each of these problems renders standard practices in fair ML unsuited to the regulatory context. 
% These problems pose significant obstacles to the use of FairML methods in model testing and auditing procedures.
Building on the literature for sensitivity analysis in FairML we turn to tools from causal inference to develop a general framework for automated sensitivity analysis in FairML settings. 
Using this framework auditors can flexibly specify different kinds and combinations of measurement bias they are worried about in their setting along with other domain specific assumptions and conduct a sensitivity analysis. This is a significant leap forward in the possibilties for sensitivity analysis in FairML.
% We conduct empirical analyses on FairML benchmark datasets, 
% demonstrating that the issues we raise are not merely theoretical: 
% many outwardly “fair” models are \textit{fragile}. 
% Under even small amounts of biases (i)--(iii),
% models can appear to exhibit negligible disparities
% despite the presence of yawning disparities %that are revealed 
% once these biases are taken into account.% Models that appear to exhibit negligible disparity 
% under the assumptions implicit in standard practice 
% reveal gross disparities when these assumptions are even mildly violated. 
% Our analysis further reveals that different classes of parity metrics
% are differentially sensitive to different kinds of bias. 
% Our testing toolkit, grounded in causal sensitivity analysis, 
% will allow regulators to understand how these dynamics
% might unfold in particular deployment circumstances.

% and with respect to particular parity measures.

% Using tools from causal inference, we develop a general sensitivity analysis framework that regulators can employ to understand how robust their parity evaluations are to various statistical biases. We conduct empirical analyses on fair ML benchmark datasets, demonstrating that the issues we raise are not merely theoretical: many seemingly fair ML models are \textit{fragile}. Models which appear to exhibit negligible disparity under the assumptions implicit in standard practice reveal gross disparities when these assumptions are even mildly violated. Our analysis further reveals that different classes of parity metric are differentially sensitive to different kinds of bias. Our testing toolkit, grounded in causal sensitivity analysis, will allow regulators to understand how these dynamics unfold in particular deployment circumstances and with respect to particular parity measures.


    
\end{abstract}
